Toward alternative metrics of journal impact: A comparison of download and citation data

We generated networks of journal relationships from citation and download data, and determined journal impact rankings from these networks using a set of social network centrality metrics. The resulting journal impact rankings were compared to the ISI IF. Results indicate that, although social network metrics and ISI IF rankings deviate moderately for citation-based journal networks, they differ considerably for journal networks derived from download data. We believe the results represent a unique aspect of general journal impact that is not captured by the ISI IF. These results furthermore raise questions regarding the validity of the ISI IF as the sole assessment of journal impact, and suggest the possibility of devising impact metrics based on usage information in general.

==> centrpics/centrall.tex <==

\setlength{\unitlength}{2000sp}

\begin{picture}(4565,2915)(3306,-5606)

% VERTICES
\put(5401,-5161){\circle{874}}
\put(5260,-5220){$v_1$}
\put(7426,-4261){\circle{874}}
\put(7280,-4261){$v_i$}
\put(3751,-4186){\circle{874}}
\put(3619,-4220){$v_3$}
\put(5401,-3136){\circle{874}}
\put(5260,-3160){$v_2$}
\put(9451,-4261){\circle{874}}
\put(9380,-4270){$v_4$}

% EDGES
%\put(5840,-5011){\vector(2,1){1160}}
\put(7010,-4470){\vector(-2,-1){1160}}


\put(4960,-5011){\vector(-3,2){830}}
\put(4070,-3866){\vector(3,2){890}}
\put(5401,-4711){\vector(0,1){1125}}
\put(7879,-4261){\vector(1,0){1115}}

% EDGE LABELS

\put(6376,-5011){$w_{i,1}$}
\put(4700,-4550){$w_{2,1}$}
\put(4050,-3386){$w_{2,3}$}
\put(3976,-5011){$w_{1,3}$}
\put(6376,-3361){$d_{i,2}$}
\put(6100,-4000){$d_{i,3}$}
\put(8200,-4000){$w_{i,4}$}


% DOTTED ARROWS
\multiput(5955,-3338)(105,-52){10}{\circle{10}}
\put(7051,-3886){\vector( 2,-1){0}}
\put(5851,-3286){\vector(-2, 1){0}}

\multiput(4405,-4186)(105,0){24}{\circle{20}}
\put(4250,-4186){\vector(-1,0){0}}
\put(6940,-4190){\vector(1,0){0}}

\end{picture}



==> pics/citgraph/citgraph2.tex <==
%\documentclass[pdftex]{article}
%\usepackage{amssymb}
%\usepackage{bez123}

%\begin{document}

\setlength{\unitlength}{2000sp}
\begin{picture}(8968,4278)(2961,-4225)

\thinlines
\put(10801,-3151){\circle{670}}
\put(11586,-1671){\circle{670}}
\put(9901,-1636){\circle{670}}

\put(4126,-1711){\circle{540}}
\put(3826,-1036){\circle{540}}
\put(5251,-2761){\circle{540}}
\put(4876,-2986){\circle{540}}
\put(5251,-3061){\circle{540}}
\put(6601,-1861){\circle{540}}
\put(6601,-2086){\circle{540}}
\put(7276,-2011){\circle{540}}
\put(7126,-1486){\circle{540}}

\put(3451,-1036){\circle{540}}
\put(4576,-3511){\circle{540}}
\put(7501,-1636){\circle{540}}
\put(4426,-1561){\circle{540}}
\put(4726,-1261){\circle{540}}

%\put(4051,-1036){\circle{4000}}
%\put(5101,-3136){\circle{4000}}
%\put(7051,-1636){\circle{4000}}

\thinlines
\cbezier[20](2851,-1036)(2851,-373.25830024)(3388.25830024,164)(4051,164)
\cbezier[20](4051,164)(4713.74169976,164)(5251,-373.25830024)(5251,-1036)
\cbezier[20](5251,-1036)(5251,-1698.74169976)(4713.74169976,-2236)(4051,-2236)
\cbezier[20](4051,-2236)(3388.25830024,-2236)(2851,-1698.74169976)(2851,-1036)

\cbezier[20](3901,-3136)(3901,-2473.25830024)(4438.25830024,-1936)(5101,-1936)
\cbezier[20](5101,-1936)(5763.74169976,-1936)(6301,-2473.25830024)(6301,-3136)
\cbezier[20](6301,-3136)(6301,-3798.74169976)(5763.74169976,-4336)(5101,-4336)
\cbezier[20](5101,-4336)(4438.25830024,-4336)(3901,-3798.74169976)(3901,-3136)

\cbezier[20](5851,-1636)(5851,-973.25830024)(6388.25830024,-436)(7051,-436)
\cbezier[20](7051,-436)(7713.74169976,-436)(8251,-973.25830024)(8251,-1636)
\cbezier[20](8251,-1636)(8251,-2298.74169976)(7713.74169976,-2836)(7051,-2836)
\cbezier[20](7051,-2836)(6388.25830024,-2836)(5851,-2298.74169976)(5851,-1636)


%\put(6976,-3886){\makebox(1.6667,11.6667){}}

\thicklines
\put(8451,-2761){\vector( 1, 0){900}}

\thinlines
\put(4270,-2040){\vector( 2,-3){450}}
\put(4576,-1786){\vector( 1,-4){225}}
\put(4801,-1561){\vector( 1,-3){300}}
\put(5551,-2611){\vector( 2, 1){750}}
\put(6301,-1711){\vector(-4, 1){1200}}
\put(10051,-1936){\vector( 2,-3){600}}
\put(10951,-2836){\vector( 2, 3){600}}
\put(11251,-1636){\vector(-1, 0){975}}


% labels
\put(3580,-261){journal}
\put(3980,-486){$v_1$}
\put(6626,-811){journal}
\put(6926,-1036){$v_2$}
\put(4900,-3886){journal}
\put(5200,-4111){$v_3$}

%\put(3151,-1486){articles}
\put(6800,-2561){articles}
%\put(5401,-3511){articles}
\put(5326,-1261){citations}
\put(6376,-4030){citation graph}
\put(10351,-4030){journal graph}

% symbols
\put(9751,-1670){$v_1$}
\put(11470,-1670){$v_2$}
\put(10650,-3180){$v_3$}

\put(9900,-2536){$3$}
\put(11551,-2536){$1$}
\put(10700,-1390){$1$}

\end{picture}

%\end{document}


==> pics/citgraph/global_local.tex <==
%\documentclass[pdftex]{article}
%\usepackage{amssymb}
%\usepackage{bez123}

%\begin{document}


\setlength{\unitlength}{2000sp}

\begin{picture}(2775,2309)(826,-2535)

%%% SMALL LOCAL CIRCLE
\put(3200,-1900){DL user community}
\put(2800,-2000){\circle{700}}
\put(2950,-2100){\vector( 3,-2){450}}
\put(3500,-2611){local impact}

%%% BIG ISI circle
\cbezier(792,-1486)(792,-887.3233312168)(1277.3233312168,-402)(1876,-402)
\cbezier(1876,-402)(2474.6766687832,-402)(2960,-887.3233312168)(2960,-1486)
\cbezier(2960,-1486)(2960,-2084.6766687832)(2474.6766687832,-2570)(1876,-2570)
\cbezier(1876,-2570)(1277.3233312168,-2570)(792,-2084.6766687832)(792,-1486)

\put(2700,-620){ISI authors}
\put(1500,-1100){ISI IF}
\put(1200,-1600){global}
\put(1200,-2000){impact}
\end{picture}

%\end{document}


==> pics/taxonomy/taxonomy.tex <==
\setlength{\unitlength}{3000sp}

\begin{picture}(3622,3144)(2101,-3361)

\thinlines
\put(3031,-1286){\framebox(900,425){}}
\put(3181,-1166){ISI IF}
\put(4636,-1286){\framebox(615,425){}}
\put(4756,-1166){RF}
\put(4621,-2411){\framebox(595,375){}}
\put(4741,-2281){SR}
\put(3000,-2261){\framebox(550,375){}}
\put(3091,-2141){SA}
\put(2450,-2696){\framebox(1570,380){}}
\put(2536,-2606){Webometrics}

\thicklines
\put(4201,-361){\vector( 0, 1){  0}}
\put(4201,-361){\vector( 0,-1){2600}}
\put(2701,-1661){\vector(-1, 0){  0}}
\put(2701,-1661){\vector( 1, 0){3000}}

\put(3601,-261){Frequency}
\put(5900,-1740){Readers}
\put(1600,-1740){Authors}
\put(3750,-3161){Structure}
%\put(2300,-2951){webmetrics}

\end{picture}

